Domain Randomization for Sim2real Transfer of Automatically Generated Grasping Datasets

Robotic grasping refers to making a robotic system pick an object by applying forces and torques on its surface. Many recent studies use data-driven approaches to address grasping, but the sparse reward nature of this task made the learning process challenging to bootstrap. To avoid constraining the operational space, an increasing number of works propose grasping datasets to learn from. But most of them are limited to simulations. The present paper investigates how automatically generated grasps can be exploited in the real world. More than 7000 reach-and-grasp trajectories have been generated with Quality-Diversity (QD) methods on 3 different arms and grippers, including parallel fingers and a dexterous hand, and tested in the real world. Conducted analysis on the collected measure shows correlations between several Domain Randomization-based quality criteria and sim-to-real transferability. Key challenges regarding the reality gap for grasping have been identified, stressing matters on which researchers on grasping should focus in the future. A QD approach has finally been proposed for making grasps more robust to domain randomization, resulting in a transfer ratio of 84% on the Franka Research 3 arm.

==> tex_files/figures/sim2real_identification_pipeline.tex <==

%\begin{figure*}[thpb]
%  \centering
%  \includegraphics[scale=1.0]{assets/diag_quality_crit.drawio.pdf}
%  \caption{\textbf{Overall approach.} A set $S$ of grasping trajectories $\tau_i$ is generated in simulation with a QD algorithm \cite{huber2023quality}. A set of $C$ quality metrics $q_{i,j}$ are then computed in simulation for each $\tau_i$. The sim2real transferability $y_i^{sim2real}$ is then measured on real robot, allowing to identify correlations between the $q_{j}$ criteria and the measured transferabilities $\hat{y}^{sim2real}$.}
%  \label{fig:identifcation_pipeline}
%\end{figure*}


% À condenser en un carré sur une colonne.



\begin{figure}[H]
  \centering
  \includegraphics[scale=1.0]{assets/sim2real_overall_principle_4.drawio.pdf}
  \caption{\textbf{Overall approach.} A set of grasping trajectories is generated in simulation with a QD algorithm \cite{huber2023quality}. Each grasp are tested into the real world, providing labels for the regression model. Quality criteria are computed in simulation. Result model predicts the probability for a given generated grasp to successfully transfer on a real robot.}
  \label{fig:identifcation_pipeline}
\end{figure}


==> tex_files/intro_tmp.tex <==


%------------------------------%
\cite{wangdemograsp}
Grasping refers to making an agent solidarize its end effector with an object by applying forces and torques on its surface. This task is of great interest in the robotics research community, as it is considered a prerequisite for many manipulation tasks (\cite{hodson2018gripping}). After the early ages of analytical-based methods (\cite{nguyen1988constructing}), data-driven approaches have dominated the literature on grasping in robotics since the beginning of the 21st century (\cite{zhang2022robotic}). Despite the involved research efforts, \textbf{grasping is still partially solved}: the reward sparsity of grasping makes it very challenging to generate data to bootstrap learning from. Consequently, most of the approaches constrain the operational space to top-down movements (\cite{yang2023pave}) or are limited to parallel grippers (\cite{fang2020graspnet}). As the self-supervised acquisition of data is very expensive (\cite{levine2018learning}), most of the recent works on grasping rely on human-provided demonstrations (\cite{wangdemograsp}, \cite{mosbach2023learning}). These promising results are at the cost of human-provided demonstrations, which is time expensive. 

To overcome this issue, Huber et al. \cite{huber2023quality} proposed to leverage Quality Diversity (QD) to generate large set of grasping trajectories. QD methods are evolutionary algorithms that optimize both quality and diversity to generate large set of high performing solution to a given problem \cite{cully2022quality}. Those methods are well known for the exploratory capabilities \cite{doncieux2019novelty}. By leveraging the well-known exploratory capabilities of QD methods, In this paper, \cite{huber2023quality} demonstrated that the well-known exploratory capabilities of QD methods could be used to generate grasping demonstrations for different end effectors, including parallel grippers and dexterous hands. Nevertheless, these results are limited to simulated scenes; exploiting such datasets into the real world would require an estimation of sim2real transferability for a given generated trajectory.

This work studies how automatically generated grasping trajectories can be transferred into the real world. The provided contributions are the following:

\begin{itemize}
    \item We have generated and deployed about N grasping grasping trajectories on M robotic platforms to target J objects to grasp, measuring the sim2real transferability associated to each of them;
    \item We investigate the correlation of K quality criteria computed in simulation with the sim2real transferability;
    \item We extensively discuss the strenghts and limitations of automatically generated grasping trajectories into the real world.
\end{itemize}

A video presenting the conducted experiments can be found online\footnote{https://youtube.com/...}. The code for generating trajectories, as well as the computation of the quality criteria, is available on Github\footnote{https://github.com/Johann-Huber/qd-grasp} – allowing roboticists to reproduce the presented results on their own platforms.

We believe this work to be a step toward the exploitation of automatically generated grasping trajectories to learn closed-loop policies that can fit specific practical needs, such as grasping quickly, cautiously, or to target a specific affordance. We also think that the ease to automatically generate demonstrations on new plateforms can contribute to alleviate the well-know reproducibility issues in the field [], spreading more easily state-of-the-art learning methods to research or industrial environments.



==> tex_files/legacy_method.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           4) Method
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\section{METHOD}
\label{sec:4_method}



%=====================================================================%
%                   2.1) Method
%=====================================================================%



%\input{tex_files/figures/sim2real_identification_pipeline}
\input{tex_files/figures/tr_me_principle}

\subsection{Overall approach}
\label{sec:4_1_overall_approach}

Fig. \ref{fig:identifcation_pipeline} describes the proposed approach to estimate sim2real transferability of automatically generated grasping trajectories. At first, a repertoire of diverse grasping trajectories is produced by a Quality-Diversity (QD) algorithm.  

...


\subsection{Quality metrics}
\label{sec:4_2_quality_metrics}


\subsubsection{Physical priors}



\subsubsection{Domain Randomization}

Domain Randomization (DR) has shown efficiency for bridging the sim-to-real gap in a wide set of robotic manipulation tasks \cite{mordotach2015ensemble}\cite{antonova2017reinforcement}\cite{enayati2023facilitating}. Many variants of DR have been experimented \cite{muratore2022robot}, but not all of them are suited to this paper topic of interest. As stated before, the QD methods are known to be fragile to stochastic domains \cite{flageat2023uncertain}. For that reason, approaches made to guide the optimization process toward solutions robust to stochasticity, such as adversarial DR \cite{zhang2021robust}, has been discarded. Plus, the sparse and binary nature of grasping reward result into limited information from real experiences – making the transferability approach of evolutionary robotics \cite{koos2012transferability} inadequate for grasping. As this work focuses on the controller generation part of grasping, vision-related DR approaches are also out of scope.

The DR approaches considered in this study involve the deployement of a trajectory to reach an object, and the application of forces on its surface. \textbf{Estimating the sim-to-real transferability of a given generated grasp can be inferred from the estimation of its robustness to perturbation of sensors, actuators and dynamics.}
The following quality criteria have therefore been proposed:
\begin{itemize}
    \item Variance of object 6DoF pose: deploying a grasp from a dataset requires to first localize the object. The 6-DoF pose estimation of objects for grasping is a largely studied problem, in which the predictions are  submitted to noise due to algorithmic approximations or sensors sensitivity [,]. In this work, we rely on a RGB-D camera, as well as a 6DoF pose estimation pipeline to localize the objects (see section []). The predicted object position is thus a source of imprecision that can increase the reality gap;
    \item Variance of joint poses: real robotic is submitted to unavoidable stochasticity caused by variations of environment's conditions (e.g. heat, humidity, joint lubricant), or wear-and-tear []. This can cause reproducibility issues that have already been discussed in the literature \cite{ibarz2021train}. Estimating the robustness to variance of joint poses is likely to provide hints on a grasping trajectory transferability;  
    \item Variance of dynamics: all simulators for learning in robotics have strengths and weaknesses, but none of them perfectly reproduce the dynamics of real experiments \cite{collins2021review}. DR on simulators dynamics have already shown promising results \cite{mordotach2015ensemble}\cite{antonova2017reinforcement}. Recently, Enayati et al. \cite{enayati2023facilitating} provided extended experimental results showing the efficiency of Real-Time Intrinsic Stochasticity (RT-IS) as DR technique. They propose the idea that RT-IS is a way to avoid the problem of parameters tuning for dynamics perturbations, arguing that the noise that come from computing hardware can mimic reality's stochasticity.   
\end{itemize}


\textit{\textbf{Application.}} Adding perturbation on sensors, actuators and simulation dynamics are often used in the DR literature, but this practice is submitted to the problem of hyperparameters tuning: a too small perturbation is not representative enough for real experiments variability, while a too large perturbation prevent the simulated agent to solve the task and acquire the targeted skill []. For applying noise of object position, we have estimated the noise of the used 6DoF object pose estimation method on the real setups, and used the measured distributions for sampling perturbations. For joint noise, we have also measure the variation of the measured joint positions throughout the generation of the same grasping trajectory several times on the real robots. Lastly, we relied on \cite{enayati2023facilitating} assumption that RT-IS fairly approximates the stochasticity of real world dynamics to use the same method, avoiding any parameter tuning for this DR criterion.


%Considering the well known gap between simulation and reality, the exploitation of datasets of QD generated grasps for real robotics requires to label them with estimation of their exploitability. more than the vision, the DR methods considered in this work involve 




% , involving perturbation of sensors, actuators, dynamics, or more sophisticated approaches like adversarial DR 

\subsubsection{Others}

...


\begin{itemize}
    \item \textit{touch\_var}: variance of touch points (obj-gripper since the end of the grasp / beginning of grasp);
    \item \textit{obj\_s\_var}: variance of obj state throughout the episode;
    \item \textit{obj\_pose\_var}: variance of obj position throughout the episode;
    \item \textit{obj\_orient\_var}: variance of obj orientation throughout the episode;
    \item \textit{robustness\_noise\_joint}: is the object still grasped after having applied noise to the joints ?
    \item \textit{robustness}: is the object still grasped after having applied noise to the object pose ?
    \item \textit{energy}: torques applied on each joint thoughout the episode;
    \item \textit{energy\_grasp}: torques applied on each joints since the beginning of grasp;
    \item \textit{energy\_post\_grasp}: torques applied on each joints since the end of grasp.
\end{itemize}

 










\subsection{Model validation}
\label{sec:4_3_model_validation}

To validate the identified model, a repertoire of grasping trajectories has been generated for each of the considered platforms. N trajectories are selected and deployed. The success rate is then measured.



==> tex_files/rw_tmp.tex <==



a QD method that generates reach-and-grasp trajectories on different robot-gripper setups. Huber et al. \cite{huber2023quality} extensively study how QD methods can efficiently generate grasping trajectories, resulting into methods that significantly outperforms NSMBS in terms of size, diversity and quality of the generated set of trajectories for different type of grippers. These results are however limited to simulations. This paper investigate how such automatically generated grasping demonstrations can be exploited into the real world by estimating their sim-to-real transferability through a regression model trained on identified quality criteria.

What distinguishes the physics-simulation-based methods from other approaches to generate grasping datasets is that the successful grasps are identified after a simulated attempt. The quality of the generated data is thus submitted to the quality of the 3D meshes that compose the scene, and the modelisation of contacts between simulated bodies. While some works propose empirical verification of the exploitability of generated data in the real world \cite{eppner2021acronym}\cite{morel2022automatic}, \textbf{the purpose of the present work is to identify metrics computed in simulated which are correlated with sim2real transferability}. Such metrics could allow practionner to rely on a finer labelling of data, associated to each generated grasp a probability to transfer – considering that learning to grasp requires larges and diverse datasets that consist of examples of different qualities. 


\cite{huber2023quality}

→ liste, taxonomie rapide
→ limites actuelles : que sur de la pince parallèle, et, malgré les nombreuses tentatives, n’a pas encore produit l’effet catalyseur pour le domaine de cherche .
→ Les algorithmes QD, une branche des méthodes évolutionnaires qui optimisent simultanément la qualité et la diversité des solutions, a été appliqué à la saisie [], démontrant la capacité de générer sur des ensembles de saisies diverses et performantes pour plusieurs bras robotiques et préhenseurs []. These results are however limited to simulations. This paper investigate how such automatically generated grasping demonstrations can be exploited into the real world by estimating their sim-to-real transferability through a regression model trained on identified quality criteria.





The interest for data-driven approaches pushes the field to produce many datasets for grasping in robotics. We can divide the literature into \textit{manually} and \textit{automatically} built datasets. Manually provided data can involve a demonstration of the overall trajectory by an expert (e.g. kinestesic [], or teleoperated []), or through image annotations (rectangle style for parallel grippers [] or pixel regions for suction grippers []). Automatically provided data can be generated through analytic methods (in simulation \cite{nguyen1988constructing}[multi fingers + regions][dexnet] or on real data point clouds \cite{fang2020graspnet}), self-supervision \cite{levine2018learning}, neuromorphic-vision based \cite{li2020event}, or relying on simulated scenes that involve a modelization of contacts. The present work is more specifically related to this last category.

The automatically generated grasping datasets based on physics simulation involves either the grasp 6-DoF poses on 3D object models \cite{kappler2015leveraging}\cite{eppner2021acronym}\cite{eppner2022billion} or the whole reach-and-grasp sequence \cite{morel2022automatic}\cite{huber2023quality}. Kappler et al. \cite{kappler2015leveraging} generates grasp poses for a 3-fingers BarrettHand by uniformly sampling approaches vectors on the simulator OpenRAVE. Eppner et al. \cite{eppner2021acronym} proposes a datasets of grasp poses for franka emika pandas parallel gripper on thousands of objects by testing grasp positions in the FleX simulator. This work has been extended to a restricted number of objects, but with about 1 billion of grasp positions overall \cite{eppner2022billion}. Contrary to these methods, Morel et al. \cite{morel2022automatic} proposes NSMBS, a QD method that generates reach-and-grasp trajectories on different robot-gripper setups. Huber et al. \cite{huber2023quality} extensively study how QD methods can efficiently generate grasping trajectories, resulting into methods that significantly outperforms NSMBS in terms of size, diversity and quality of the generated set of trajectories.

What distinguishes the physics-simulation-based methods from other approaches to generate grasping datasets is that the successful grasps are identified after a simulated attempt. The quality of the generated data is thus submitted to the quality of the 3D meshes that compose the scene, and the modelisation of contacts between simulated bodies. While some works propose empirical verification of the exploitability of generated data in the real world \cite{eppner2021acronym}\cite{morel2022automatic}, \textbf{the purpose of the present work is to identify metrics computed in simulated which are correlated with sim2real transferability}. Such metrics could allow practionner to rely on a finer labelling of data, associated to each generated grasp a probability to transfer – considering that learning to grasp requires larges and diverse datasets that consist of examples of different qualities. 

  
% Peut-être mélanger 2 et 3 : "Grasp quality and sim2real transferability






% --------

The \textit{reality gap} describes the large difference between simulated robotics scenes and real ones, preventing to reproduce results from simulation into the real world \cite{salvato2021crossing}. The reality gap is still one of the critical problems that make real-world grasping so challenging \cite{zhang2022robotic}. Many methods have been proposed to reduce this phenomenon, including system identification [], domain adaptation [] and domain randomization [].



% \cite{tobin2017domain}\cite{khosla2020supervised}.

%iterative learning control, employs real-world data to improve the dynamics model used to determine the optimal control behavior, rather than using real-world data to improve the controller directly.


% Some previous works did experimental measures to 

% Collins et al. mesure the differences between several simulators and real sensors to quantify reality gap \cite{collins2019quantifying},

% On the acquisition of large amount of sim2real data, [] is a database of self-supervised datasets. For each data, a label that describe the success of the attempt is provided. While provinding a very large sim2real dataset, A limitat


%...
% reality gap : well know problem in robotics
% some specific methods have been proposed to specifically reduce it \bibitem{tobin2017domain}\bibitem{khosla2020supervised}
% 

% TODO: un peu de biblio pour se positionner plus précisément


















%----------------





The most commonly used quality metric is the force closure criteria of Nguyen et al. \cite{nguyen1988constructing}. Many works rely on it to label sampled grasps from point cloud [graspnet], usually based on the Graspit! [] (e.g. [dexnet]). Recent work exploit data-driven approaches with this metrics to compute a robustness score \cite{liang2019pointnetgpd}(à vérifier). While relying on solid mathematical proofs, force closure is a solid criterion in simulation – but it is not a universal panacea: if the meshes of the 3D object model does not match the reality, a considered grasp pose might results into a failure in the real world.

Recent works rely on different approaches than analytic based ones for labeling quality of grasps. Ottenhaus et al. \cite{ottenhaus2019visuo} train a deep-learning model to predict the force-closure probability under small perturbations. Varley et al. \cite{varley2015generating} learn heatmaps of grasp efficiency based on grasp pose... ? Wen et al. assumes that « the stability of a grasp should be continuous in the neighborhood of a 6DoF pose» to estimate a robustness score by measuring the stability of randomly sampled poses close to the considered grasp \cite{wen2022catgrasp}.

Overall, there is no consensus on the notion of grasp quality in the literature. Some recent works even mention the need for explicitly stating what a \textit{successful} grasp is, as its binary nature can hide different levels of robustness.

% In addition to reporting the grasp success rate, researchersshould consider reporting a more strict definition of the grasp success that tests the robustness of the grasp, similar to Lundell et al.

%Def prposée : the quality associated with a grasp is the probability for this grasp to succeed. 
% Thus, the sim2real quality is the probability for a successful simulated grasp to succeed into the real world.

